Semantic Segmentation Prior for Diffusion-Based Real-World Super-Resolution

Real-world image super-resolution (Real-ISR) has achieved a remarkable leap by leveraging large-scale text-to-image models, enabling realistic image restoration from given recognition textual prompts. However, these methods sometimes fail to recognize some salient objects, resulting in inaccurate semantic restoration in these regions. Additionally, the same region may have a strong response to more than one prompt and it will lead to semantic ambiguity for image super-resolution. To alleviate the above two issues, in this paper, we propose to consider semantic segmentation as an additional control condition into diffusion-based image super-resolution. Compared to textual prompt conditions, semantic segmentation enables a more comprehensive perception of salient objects within an image by assigning class labels to each pixel. It also mitigates the risks of semantic ambiguities by explicitly allocating objects to their respective spatial regions. In practice, inspired by the fact that image super-resolution and segmentation can benefit each other, we propose SegSR which introduces a dual-diffusion framework to facilitate interaction between the image super-resolution and segmentation diffusion models. Specifically, we develop a Dual-Modality Bridge module to enable updated information flow between these two diffusion models, achieving mutual benefit during the reverse diffusion process. Extensive experiments show that SegSR can generate realistic images while preserving semantic structures more effectively.

==> figs/tex/fig_zeromap.tex <==
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{Metrics} & \multicolumn{2}{c}{DIV2K-Val} & \multicolumn{2}{c}{RealSR} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & Zero Mask & SegSR & Zero Mask & SegSR \\
\midrule
PSNR $\uparrow$ & 20.26 & 20.42 & 24.55 & 24.61 \\
SSIM $\uparrow$ & 0.4448 & 0.4659 & 0.6774 & 0.6858 \\
LPIPS $\downarrow$ & 0.4026 & 0.3769 & 0.3370 & 0.3434 \\
DISTS $\downarrow$ &0.2407 & 0.2240 & 0.2398 & 0.2349 \\
MUSIQ $\uparrow$ & 69.36 & 72.29 & 64.75 & 67.80 \\
MANIQA $\uparrow$ & 0.4715 & 0.6006 & 0.4387 & 0.5233 \\
CLIPIQA $\uparrow$ & 0.6917 & 0.7723 & 0.6221 & 0.6906 \\
\bottomrule
\end{tabular}}
\caption{Metrics comparison on DIV2K-Val and RealSR datasets.}
\label{tab:zero}
\end{table}


\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/paper/zeromap.pdf}
    \caption{We present the final result predictions at different steps $t$ of the inverse diffusion process, comparing the outcomes using the all-zero mask (top) and our enhanced mask (bottom).}
    \label{fig:zeromap}
\end{figure*}

==> figs/tex/seg2img.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/paper/seg2img.pdf}
    \caption{Controlling Stable Diffusion~\cite{sd} with segmentation embedding from SegDM. The third column is the segmentation predictions of SegDM on the LQ images. The last column shows images generated under the guidance of semantic segmentation.}
    \label{fig:s2i}
\end{figure}

==> figs/tex/supp_more_fig.tex <==
\def\fwidth{0.16\linewidth}
\def\arraystretch{0.5}
\renewcommand{\tabcolsep}{0.5 pt}
\begin{figure*}[!ht]
\centering
\begin{tabular}{ccccc}
    % \centering{\rotatebox{90}{  \small{DIV2K-810}}}  \hspace{1pt} &
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/LQ.png} &  
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/bsrgan.png} &  
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/realesrgan.png} &  
    % % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/dasr.png} & 
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/stablesr.png} &  
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/resshift.png} &  
    % % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/pasd.png} & 
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/diffbir.png} & 
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/seesr.png} &  
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/SegSR.png} &
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/810_color_rect_resize/HQ.png} 
    % \\ 
     % \centering{\rotatebox{90}{  \small{DIV2K-844}}}  \hspace{1pt} &
    \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/LQ_x4.png} &  
    \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/bsrgan.png} &  
    \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/realesrgan.png} &  
    % \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/dasr.png} & 
    \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/resshift.png} &
     \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/stablesr.png} 
    \\ 
       \small{LQ}
    &   \small{BSRGAN}
    &   \small{Real-ESRGAN}
    % &   \small{DASR}
    &   \small{ResShift}
    &   \small{StableSR}
    \\

    \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/diffbir.png} & 
    \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/pasd.png} & 
    \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/seesr.png} &  
    \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/SegSR.png} &
    \includegraphics[width=\fwidth]{figs/results/div2k-val/852_rect_resize/HQ.png} 
    \\
    % &   \small{StableSR}
     \small{DiffBIR}
    &   \small{PASD}
    &   \small{SeeSR}
    &   \small{\textbf{SegSR}}
    &   \small{HQ}
\end{tabular}
\caption{Qualitative comparisons on synthetic benchmark DIV2K-Val~\cite{div2k}. Please zoom in for details.}
\label{fig:qualitative_supp_div2k}
\end{figure*}

\renewcommand{\tabcolsep}{5 pt}

==> figs/tex/supp_more_fig_real.tex <==

\def\fwidth{0.16\linewidth}
\def\arraystretch{0.5}
\renewcommand{\tabcolsep}{0.5 pt}
\begin{figure*}[!ht]
\centering
\begin{tabular}{ccccc}
  
    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/LQ_x4.png} &  
    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/bsrgan.png} &  
    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/realesrgan.png} &  
    % \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/dasr.png} &  
    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/resshift.png}  & 
    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/stablesr.png} 
        \\ 
       \small{LQ}
    &   \small{BSRGAN}
    &   \small{Real-ESRGAN}
    % &   \small{DASR}
    &   \small{ResShift}
    &   \small{StableSR}
    \\


    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/diffbir.png} & 
    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/pasd.png} & 
    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/seesr.png} &  
    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/SegSR.png} &
    \includegraphics[width=\fwidth]{figs/results/ost-val/165_rect_resize/HQ.png} 
     \\ 
     \small{DiffBIR}
    &   \small{PASD}
    &   \small{SeeSR}
    &   \small{\textbf{SegSR}}
    &   \small{HQ}
    % \\ 
    % \\ 
    % \centering{\rotatebox{90}{  \small{OST}}}  \hspace{1pt} &
    % \includegraphics[width=\fwidth]{eccv/icvl_rect_resize/gt.png} &  
    % \includegraphics[width=\fwidth]{eccv/icvl_big/noise.png} &  
    % \includegraphics[width=\fwidth]{eccv/icvl_big/macnet.png} &  
    % \includegraphics[width=\fwidth]{eccv/icvl_big/t3sc.png} & 
    % \includegraphics[width=\fwidth]{eccv/icvl_big/mst.png} &  
    % \includegraphics[width=\fwidth]{eccv/icvl_big/sst.png} &  
    % \includegraphics[width=\fwidth]{eccv/icvl_big/sert.png} & 
    % \includegraphics[width=\fwidth]{eccv/icvl_big/hsdt.png} & 
    % \includegraphics[width=\fwidth]{eccv/icvl_big/s2s.png} &  
    % \includegraphics[width=\fwidth]{eccv/icvl_big/s2s.png} &  
    % \includegraphics[width=\fwidth]{eccv/icvl_big/gt.png} 
    % \\ 
   
    %  \rotatebox{90}{  \small{RealPhoto60}} \hspace{1pt} &
    % \includegraphics[width=\fwidth]{eccv/wdc_rect_resize/gt.png} &  
    % \includegraphics[width=\fwidth]{eccv/wdc_big/noisy.png} &  
    % \includegraphics[width=\fwidth]{eccv/wdc_big/macnet.png} &  
    % \includegraphics[width=\fwidth]{eccv/wdc_big/T3SC.png} & 
    % \includegraphics[width=\fwidth]{eccv/wdc_big/mst.png} & 
    % \includegraphics[width=\fwidth]{eccv/wdc_big/sst.png} &
    % \includegraphics[width=\fwidth]{eccv/icvl_big/s2s.png} &  
    % \includegraphics[width=\fwidth]{eccv/wdc_big/sert_base.png} &  
    % \includegraphics[width=\fwidth]{eccv/wdc_big/hsdt.png} & 
    % \includegraphics[width=\fwidth]{eccv/wdc_big/s2s.png} &  
    % \includegraphics[width=\fwidth]{eccv/wdc_big/gt.png} 
    % \\
    % \centering{\rotatebox{90}{  \small{RealLQ250}}}  \hspace{1pt} &
    % \includegraphics[width=\fwidth]{eccv/real_rect_resize/noise.png} &  
    % \includegraphics[width=\fwidth]{eccv/real_big/noise.png} &  
   
    % \includegraphics[width=\fwidth]{eccv/real_big/macnet.png} &  
    % \includegraphics[width=\fwidth]{eccv/real_big/T3SC.png} & 
    % \includegraphics[width=\fwidth]{eccv/real_big/mst.png} &  
    % \includegraphics[width=\fwidth]
    % {eccv/real_big/sst.png} &  
    % \includegraphics[width=\fwidth]{eccv/real_big/sert_base.png} & 
    % \includegraphics[width=\fwidth]{eccv/real_big/hsdt.png} & 
    % \includegraphics[width=\fwidth]{eccv/real_big/s2s.png} &
    % \includegraphics[width=\fwidth]{eccv/real_big/s2s.png} &
    % \includegraphics[width=\fwidth]{eccv/real_big/gt.png} 
\end{tabular}
\caption{Qualitative comparisons on synthetic benchmark OST-Val~\cite{sftgan}. Please zoom in for details.}
\label{fig:qualitative_supp_ost}
\end{figure*}

\def\fwidth{0.16\linewidth}
\def\arraystretch{0.5}
\renewcommand{\tabcolsep}{0.5 pt}
\begin{figure*}[!ht]
\centering
\begin{tabular}{ccccc}

    \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/LQ_x4.png} &  
    \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/bsrgan.png} &  
    \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/realesrgan.png} &  
    \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/dasr.png} & 
    \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/resshift.png} 
        \\ 
       \small{LQ}
     & \small{BSRGAN}
    &   \small{Real-ESRGAN}
    &   \small{DASR}
    &   \small{ResShift}
    \\
     \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/stablesr.png} & 
    \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/diffbir.png} & 
    \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/pasd.png} & 
    \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/seesr.png} &  
    \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/SegSR.png} \\
    % \includegraphics[width=\fwidth]{figs/results/realsr-128/nikon_047_color_rect_resize/HQ.png} 

       \small{StableSR}
    &  \small{DiffBIR}
    &   \small{PASD}
    &   \small{SeeSR}
    &   \small{\textbf{SegSR}}
    % &   \small{HQ}
\end{tabular}
\caption{Qualitative comparisons on real-world benchmark RealSR~\cite{realsr}. Please zoom in for details.}
\label{fig:qualitative_supp_realsr}
\end{figure*}


\def\fwidth{0.16\linewidth}
\def\arraystretch{0.5}
\renewcommand{\tabcolsep}{0.5 pt}
\begin{figure*}[!ht]
\centering
\begin{tabular}{ccccc}

       \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/LQ_x4.png} &  
    \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/bsrgan.png} &  
    \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/realesrgan.png} &  
    \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/dasr.png} & 
    \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/resshift.png} 
        \\ 
       \small{LQ}
     & \small{BSRGAN}
    &   \small{Real-ESRGAN}
    &   \small{DASR}
    &   \small{ResShift}
    \\
     \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/stablesr.png} & 
    \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/diffbir.png} & 
    \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/pasd.png} & 
    \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/seesr.png} &  
    \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/SegSR.png} \\
    % \includegraphics[width=\fwidth]{figs/results/reallq-250/216_color_rect_resize/HQ.png} 

       \small{StableSR}
    &  \small{DiffBIR}
    &   \small{PASD}
    &   \small{SeeSR}
    &   \small{\textbf{SegSR}}
    % &   \small{HQ}
\end{tabular}
\caption{Qualitative comparisons on real-world benchmark RealLQ250~\cite{dreamclear}. Please zoom in for details.}
\label{fig:qualitative_supp_reallq}
\end{figure*}

\renewcommand{\tabcolsep}{5 pt}



==> sec/3_method_bak.tex <==
\section{Methodology}
\label{sec:method}
\input{figs/tex/framework}
\subsection{Motivation}
\label{sec:overview}
To harness the potential of pretrained T2I diffusion models, methods like PASD~\cite{pasd} and SeeSR~\cite{seesr} have successfully integrated high-level semantic prompt information as additional conditions.
%
These methods enable Real-ISR to generate images with more realistic details and improved semantic fidelity.
%
However, these prompt-based Real-ISR methods rely on multimodal language models to recognize the semantic content of images and implicitly localize semantic prompts through cross-attention, exposing two potential limitations.
% Firstly, these prompts-based methods lack detailed spatial position descriptions,  which can result in misalignment between prompts and regions in the LQ image.
%
Firstly, multimodal language models often overlook describing some salient objects in the image, leading to inaccurate restoration of semantic details in regions corresponding to those omitted objects.
%
As shown in the top row of Figure~\ref{fig:errors} (a), SeeSR fails to cover the salient object `building' and the implicit cross-attention mistakenly localizes the object `stone' to the building-styled region, causing stone-like textures to appear in the building area.
%
In addition, as shown in the bottom row of Figure~\ref{fig:errors} (a), SeeSR fails to capture salient the object `sky' or `cloud' across the image. This leads to inaccurate restoration of the zoomed area,  as cross-attention misallocates attention from the object 'mountain' to this region.
%
For the second issue, the implicit localization of cross-attention may lead to overallocate weights to irrelevant tokens within the same spatial region, confusing the model's understanding of this area and leading to semantic ambiguity in image generation.
%
As shown in Figure~\ref{fig:errors}(b), cross-attention assigns weights to both `horse' and `person' in the red-boxed area, resulting in a confusing image that blends `person' and `horse' features in this region. 
% In addition, the implicit localization of cross-attention may lead to overallocate weights to irrelevant tokens within a same spatial region, confusing the model's understanding of this area and leading to semantic ambiguous generation. As shown in Figure~\ref{fig:errors}(b), cross-attention assigns weights to both "horse" and "person" in the red-boxed area, resulting in a confusing image that blends "person" and "horse" features in this region. For the second issue, multimodal language models often prioritizes more salient objects, resulting in incomplete descriptions in high-density object scenes. Consequently, the omitted object regions lose semantic control, and cross-attention may even allocate weights from other objects to these regions. As shown in  bottom row of Figure~\ref{fig:errors}(a), The DAPE recognition module in SeeSR fails to cover the "sky" class prompt, resulting in the zoomed area not being accurately restored and misallocate the prompt of "mountain" to this region.
%

This motivates us that if we can introduce semantic segmentation into Real-ISR, which holds the potential to enable a more comprehensive perception of salient objects within the image by assigning class labels to each pixel. 
%
Additionally, it facilitates clearer semantic spatial localization and reduces the risks of semantic ambiguity by explicitly allocating objects to their respective spatial regions.
% %
% The semantic segmentation prior holds the potential to enable more comprehensive perception of salient objects within the image, while facilitating clearer semantic spatial localization and reducing the risks of semantic ambiguities.
%
% As shown in Figure~\ref{fig:errors}, our method incorporated with semantic segmentation priors can effectively address the aforementioned limitations of prompt-guided methods, generating the correct and coherent semantic content in each corresponding area. 
%
As shown in Figure~\ref{fig:errors}, our method, incorporating semantic segmentation priors, effectively addresses the aforementioned limitations of prompt-guided methods and generates accurate, coherent semantic content in each corresponding area.

However, directly predicting the pleasant segmentation results from the LQ image is challenging. As shown in Figure~\ref{fig:inter} (a), 
we use a Segformer pretrained on LQ images to predict segmentation masks that guide diffusion-based ISR model (SRDM) in restoration. However, its predictions on degraded images are often inaccurate, leading SRDM to generate incorrect semantic content in corresponding regions (e.g., generating `mountain' textures in `building' regions). 
It is worth emphasizing that improved image results and refined segmentation predictions can mutually enhance each other’s quality. This motivates us to leverage restored features from SRDM to assist semantic segmentation, while refining segmentation predictions from diffusion-based segmentor (SegDM) to enhance image restoration. Therefore, in this work, we attempt to design a mutual refinement framework that facilitates interaction in both SRDM and SegDM, ultimately achieving image restoration performance. As shown in Figure~\ref{fig:inter} (b), the
dual-diffusion mutual refinement framework can gradually restore HQ image and more accurate semantic segmentation predictions with the information interaction between the SRDM and SegDM across all steps.

\input{figs/tex/fig_inter_results}
\subsection{Framework Overview}
In this paper, we present SegSR, a semantic segmentation prior-interpolated diffusion framework designed to tackle the challenge of Real-ISR task. As shown in Figure~\ref{fig:framework}, SegSR consists of two branches, SRDM and SegDM, connected by the Dual-Modality Bridge (DMB). Among them, SRDM employs the architecture of StableSR to generate realistic restored images based on the conditions of the LQ image. SegDM is a discrete diffusion model that gradually predicts the segmentation mask from the given LQ image. As for DMB, it acts as a bridge connecting SRDM and SegDM, based on the premise that improved mask predictions can enhance the realism of SRDM-generated images, while higher-quality SR images also aid in better mask prediction. During the diffusion process, it provides updated segmentation priors to SRDM and iteratively restored image information to SegDM. More detailed information about these modules is as follows:



\begin{itemize}
    \item For the SRDM branch, we adopt StableSR~\cite{stablesr} as the baseline for Real-ISR tasks where the trainable modules include the image controller (i.e., Time-aware Encoder) and the SFT layer~\cite{sftgan} that integrates the LQ image's representation embedding into Img Denoiser (i.e., denoising UNet in SD).
    \item  For the SegDM branch,  we adopt the structure of DDPS~\cite{ddps} for segmentation prior to modeling. It consists of a Seg Backbone and a Seg Denoiser. The Seg Backbone utilizes the backbone of Segformer as the image feature extractor, while the Seg Denoiser employs a variant of U-Net~\cite{unet} to eliminate noise during the diffusion process. The image features derived from the backbone are conditionally fed into the Seg Denoiser to enhance the accuracy of mask predictions.
    \item For the DMB module, it consists of SegControl and ImgAided modules. Specifically, SegControl follows the methodology and structure as ControlNet~\cite{controlnet}. It encodes the intermediate, updated segmentation prior from SegDM and injects it into SRDM via zero convolution. This can be considered a Seg2Img generator that produces images with the corresponding spatial semantic content defined by the segmentation prior. The ImgAided component leverages a lightweight U-Net~\cite{sd}, which encodes the iteratively restored image latent from SRDM and uses zero convolution to introduce it into SegDM's Seg-Denoiser, enabling clearer image information to contribute to the improvement of segmentation quality. 
\end{itemize}

% \subsection{Training of SegDM Branch}
% % {\flushleft\textbf{Training of SegDM Branch.}}\quad
% we expect to predict precise semantic segmentation mask from the LQ image to facilitate the SR process for generating semantics-layout faithful Real-ISR results. To achieve this, we develop SegDM and the training of SegDM goes through two stages. In the first stage, we train a degradation-aware Segformer, consisting of a backbone and a segmentation head, expected to predict coarse segmentation masks on LQ images that approximate the ground-truth masks from HR images.
% Thus, we force the mask predictions from the LQ images to be close to that of the HR masks.
% In the second stage, inspired by DDPS~\cite{ddps}, we train a discrete diffusion model, i.e., SegDM, to capture the distribution of ground-truth (GT) mask prior.  Similar to the image process in SD, the GT mask is encoded into representation $S_0$ by a Seg Encoder, i.e, a simple resize codec, and then progressively added noise by following $t$ diffusion steps to $S_0$ to obtain the noisy representation $S_t$.
% During training, Seg Denoiser iteratively denoises $S_t$ to $S_{t-1}$, conditioned on the the image features $F_{lq}$ extracted by the frozen trained Segformer's backbone from first stage, refining the coarse prediction results from the first stage. Finally, the logit output can be reconstructed by the Seg Decoder, which performs the inverse operation of the Seg Encoder. Both stages are optimized using the cross-entropy function to compute loss between logit output and GT mask, and the training objective of SegDM is formulated as follows:
% \begin{equation}
% \mathcal{L}_{SegDM}=-\log p_\theta\left(S_0\mid S_t,F_{lq}\right).
% \label{eqa:segdm}
% \end{equation}


% \subsection{Training of DMB Module}
% % {\flushleft\textbf{Training of DMB Module.}}\quad
% As the information bridge between the SRDM and SegDM branches,  the components (i.e., Seg Controller and ImgAided Module) within DMB module is first trained independently in parallel for each branch rather than jointly, to accelerate convergence and enhance model stability.

% For Seg Controller that introduces the segmentation prior into SRDM branch,  we divide the training process into two progressive stages. First, to ensure that the segmentation prior can accurately generate corresponding semantic classes and layouts, we train the Seg Controller for stable Seg2Img generation, with ControlNet~\cite{controlnet} initialized by cloning the U-Net encoder from the pre-trained SD model.
% During training, the latent embedding $Z_0$ of the HR image is obtained by the encoder of pretrained VAE~\cite{sd}. The diffusion process progressively add noise by following $t$ steps to $Z_0$ to obtain the noisy latent $Z_t$.
% Thus, with the noisy segmentation embedding $S_t$, the Seg2Img generator $\epsilon_\theta^1$ predict the noise $\epsilon$ added to the noisy latent $Z_t$. the training objective $\mathcal{L}_{Seg2Img}$ is formulated as follows:
% \begin{equation}
% \mathcal{L}_{Seg2Img}=\mathbb{E}_{t,Z_0, S_t,\epsilon\sim\mathcal{N}}\Big[\|\epsilon-\epsilon_\theta^{1}(Z_t,t,S_t))\|_2^2\Big].
% \end{equation}

% Next, the learned Seg Controller is copied to the second stage for incorporating segmentation prior into the SR process.  For the SRDM branch, we employ the StableSR~\cite{stablesr} as the baseline, leveraging its pre-trained model in conjunction with the trained Seg Controller for joint optimization. Specifically, similar to the HQ latent $Z_0$, LQ images are processed through the Img Encoder (VAE~\cite{sd}) to derive the LQ latent $Z_{lq}$. This latent $Z_{lq}$ is then fed into the Img Controller (Time-aware Encoder) to obtain the LQ feature condition, which is integrated into the SD for generation guidance via a trainable SFT layer~\cite{sftgan}. 
% Therefore, compared to the first stage, the introduction of the additional LQ latent condition $Z_{lq}$ modifies the joint optimization objective of whole network $\epsilon_\theta^{2}$ to $\mathcal{L}_{SR}$:
% \begin{equation}
% \mathcal{L}_{SR}=\mathbb{E}_{t,Z_0, S_t,Z_{lq},\epsilon\sim\mathcal{N}}\Big[\|\epsilon-\epsilon_\theta^{2}(Z_t,t,S_t,Z_{lq}))\|_2^2\Big].
% \end{equation}

% For ImgAided Module, we train it together with  the  frozen pre-trained SegDM branch for incorporating the restored image information into segmentation prediction. 
% In specific, we pass the noisy latent $Z_t$ at $t$ step through the randomly initialized ImgAided Module to obtain the SR-aided feature, which is added to the input of Seg Denoiser.
% Thus, similar to the training objective of SegDM at Eq.~\ref{eqa:segdm}, the ImgAided Module is trained using noisy image latent $Z_t$:
% \begin{equation}
% \mathcal{L}_{IAM}=-\log p_\theta\left(S_0\mid S_t,F_{lq},Z_t \right).
% % \label{eqa:iam}
% \end{equation}


\subsection{Dual-Diffusion Mutual Refinement}
As discussed in the subsection~\ref{sec:overview},   
traditional segmentors fail to generate pleasant results when handling severe degradation, and SRDM is unable to restore HQ images with semantic fidelity when the segmentation priors are inaccurate. 
In this subsection, we present a dual-diffusion mutual refinement framework (SegSR) to facilitate interaction between image restoration and semantic segmentation at each diffusion step. It consists of two branches, SRDM and SegDM, connected by the Dual-Modality Bridge (DMB). 

As illustrated in~\cite{ddm}, diffusion models can model not only image distributions but also discrete data, such as semantic segmentation masks. Thus, similar to~\cite{ddps}, we adopt the discrete diffusion model to model the ground truth mask prior (i.e., SegDM). Following the Markov chain of the diffusion process, the GT segmentation mask is encoded as $S_0$ via a simple resize codec, progressively adding noise over $t$ steps to reach the noisy state $S_t$. Then, SegDM uses the Seg Denoiser to remove noises from $S_t$ and generate $S_{t-1}$, guided by initial predictions $F_{lq}$ from Segformer. This iterative refinement process better aligns Segformer’s predictions with the GT mask distribution.
To improve the consistency of segmentation predictions with the semantics of the input image, $I_t$, containing restored image information estimated by DMB, is incorporated into the input of the Seg Denoiser. SegDM leverages both segmentation prior modeling and restored image condition guidance, generating more semantically consistent segmentation aligned with the LQ image.

As semantic segmentation can benefit image restoration and vice versa, we
propose a Dual-modality Bridge (DMB) for joint optimization. DMB consists of SegControl and ImgAided modules. The ImgAided module at time step $t$ first extracts restored image information from $Z_t$
% {\flushleft\textbf{Training of SRDM Branch}}\quad
% For the SRDM branch, we employ the StableSR~\cite{stablesr} as the baseline, leveraging its pre-trained model in conjunction with the Seg Controller within DMB module for joint optimization.
% The Seg Controller initialized by cloning the U-Net encoder from the pre-trained SD model.
% During training, the Seg Controller receives the updated segmentation result $S_t$ from SegDM at $t$ step as input and outputs the Seg feature $C_t$, while the Img Controller (Time-aware Encoder) receives the LQ image latent $Z_{lq}$ to obtain the LQ feature condition, where $S_t$ is detailed in section of Training of SegDM Branch and $Z_{lq}$ is obtained through the Img Encoder (VAE~\cite{sd}) processing LQ image.
% Then,  the Seg feature $C_t$ and LQ feature condition are introduced into the Img Denoiser of SRDM via zero convolution and SFT layers~\cite{sftgan}, respectively. 
% Similar to SD training process, the latent embedding $Z_0$ of the HQ image is obtained by the encoder of pretrained VAE~\cite{sd}, and the diffusion process progressively add noise by following $t$ steps to $Z_0$ to obtain the noisy latent $Z_t$. Thus, the SRDM $\epsilon_\theta$ predict the noise $\epsilon$ added to the noisy latent $Z_t$:
% \begin{equation}
% \mathcal{L}_{SR}=\mathbb{E}_{t,Z_0, S_t,Z_{lq},\epsilon\sim\mathcal{N}}\Big[\|\epsilon-\epsilon_\theta(Z_t,t,S_t,Z_{lq}))\|_2^2\Big].
% \end{equation}
% {\flushleft\textbf{Training of SegDM Branch}}\quad
% As predicting precise semantic segmentation mask from the LQ image is changeling, the training of SegDM goes through two stages. In the first stage, we train a degradation-aware Segformer, consisting of a backbone and a segmentation head, expected to predict coarse segmentation masks on LQ images that approximate the ground-truth masks from HQ images.
% In the second stage, inspired by DDPS~\cite{ddps}, we train a discrete diffusion model to capture the distribution of semantic segmentation prior. During training, the GT mask is encoded into representation $S_0$ by a Seg Encoder, i.e, a simple resize codec, and then progressively added noise by following $t$ diffusion steps to $S_0$ to obtain the noisy representation $S_t$. Seg Denoiser iteratively denoises $S_t$ to $S_{t-1}$, conditioned on the the backbone features $F_{lq}$ from first stage, refining the coarse prediction results of Segformer. Finally, the logit output can be reconstructed by the Seg Decoder, which performs the inverse operation of the Seg Encoder. Both stages are optimized using the cross-entropy function to compute loss between logit output and GT mask, and the training objective of SegDM is formulated as follows:
% \begin{equation}
% \mathcal{L}_{SegDM}=-\log p_\theta\left(S_0\mid S_t,F_{lq}\right).
% \label{eqa:segdm}
% \end{equation}
% {\flushleft\textbf{Joint Training of SegSR model}}\quad
% SegSR aims to facilitate mutual refinement between SRDM and SegDM at each diffusion step. Thus, as a bridge connecting the two branches, the DMB needs to be trained jointly with both branches.
% For ImgAided Component, we pass the image latent $Z_t$ at $t$ step through it to obtain the restored image information $T_t$, which is then  added to the input of Seg Denoiser within SegDM through zero convolution to enhance segmentation prediction. 
% Thus, similar to the optimization objective of SegDM at Eq.~\ref{eqa:segdm}, the ImgAided Component is trained using noisy image latent $Z_t$:
% \begin{equation}
% \mathcal{L}_{IAC}=-\log p_\theta\left(S_0\mid S_t,F_{lq},Z_t \right).
% % \label{eqa:iac}
% \end{equation}

% For the Seg Controller, we directly copy the pretrained weights of the Seg Controller from the SRDM training stage. Thus, the joint loss function of the whole SegSR framework defined as follows:
% \begin{equation}
% \mathcal{L}_{SegSR}=\mathcal{L}_{SR}+\lambda\mathcal{L}_{IAC}.
% % \label{eqa:iam}
% \end{equation}
% where $\lambda$ is a balance parameter. The SRDM and SegDM is initialized with the pretrained weights from their respective independent training stages. For saving the training cost, the trainable modules include DMB, Time-aware Encoder and SFT layer within SRDM.

\input{figs/tex/tab_quantitative}
{\flushleft\textbf{Inference of SegSR model}}\quad
% SegSR aims to facilitate mutual refinement between SRDM and SegDM at each diffusion step. Thus, after the independent training of the DMB, we copy its pretrained weights and proceed to jointly train the whole SegSR framework, with the loss function defined as follows:
% \begin{equation}
% \mathcal{L}_{SegSR}=\mathcal{L}_{SR}+\lambda\mathcal{L}_{IAM}.
% % \label{eqa:iam}
% \end{equation}
% where $\lambda$ is a balance parameter. For saving the training cost, the trainable modules include DMB, Time-aware Encoder and SFT layer within SRDM.
After introducing SRDM, SegDM, and DMB, the sampling process of SegSR is summarized as follows. Initially, features $Z_{lq}$ and $F_{lq}$ are extracted from the LQ image using the VAE encoder and Seg backbone. The inference process follows a denoising trajectory that begins with a noisy latent representation $Z_T$ and mask $S_T$. In the SRDM branch, the Img Denoiser predicts a less noisy latent $Z_{t-1}$ based on $Z_t$, LQ features $Z_{lq}$, and segmentation prior $S_t$ from the DMB at each step. Simultaneously, the Seg Denoiser estimates the latent state of the segmentation mask $S_{t-1}$, using $S_t$ from the previous step and image condition $Z_t$ from the DMB. After $T$ collaborative diffusion steps, we estimate $Z_0$, and the VAE decoder reconstructs a high-fidelity and realistic HQ image.
Thanks to the joint optimization strategy facilitated by DMB, the proposed SegSR framework can progressively restore high-quality images through SRDM, while simultaneously improving the accuracy of semantic segmentation in SegDM, as illustrated in Figure.
